Almost Sure Convergence of Networked Policy Gradient over Time-Varying Networks in Markov Potential Games

We propose networked policy gradient play for solving Markov potential games with continuous and/or discrete state-action pairs. During the game, agents use parametrized and differentiable policies that depend on the current state and the policy parameters of other agents. During training, agents update their policy parameters following stochastic gradients. The gradient estimation involves two consecutive episodes, generating unbiased estimators of reward and policy score functions. In addition, it involves keeping estimates of others' parameters using consensus steps given local estimates received through a time-varying communication network. In Markov potential games, there exists a potential value function among agents with gradients corresponding to the gradients of local value functions. Using this structure, we prove almost sure convergence to a stationary point of the potential value function with rate $O(1/\epsilon^2)$. Compared to previous works, our results do not require bounded policy gradients or initial agreement on the values of individual policy parameters. Numerical experiments on a dynamic multi-agent newsvendor problem verify the convergence of local beliefs and gradients. It further shows that networked policy gradient play converges as fast as independent policy gradient updates, while collecting higher rewards.

==> dfp_com_aware/introduction.tex <==

%Networked systems are multi-agent structures in which agents share their information (including but not limited to observations, parameters, and actions) with each other through a communication network. Typical examples of the networked learning in multi-agent reinforcement learning (MARL) include stabilization of the joint behavior \cite{jiang2018graph}
Markov (stochastic) games describe the rational behavior of selfish decision-makers (agents) with individual rewards, depending on the joint decisions, in dynamic environments \cite{shapley1953stochastic}. Markov games are relevant models of  multi-agent autonomous systems in many settings and their solutions to related canonical problems, e.g., navigation \cite{jia2023rapid}, path planning \cite{muralidharan2019path}, and electricity demand management \cite{narasimha2022multi}. The frequent occurrence of Markov games in such systems prompt the need to design efficient algorithms for solving them. In this paper, we provide a networked multi-agent reinforcement learning (MARL) algorithm for solving Markov potential games. 


Markov potential games assume the existence of a potential value function that aligns with the changes in individual value functions which are discounted sum of rewards. If this potential value function is known by an entity that can dictate the players what to do, then the entity can solve the Markov game for a potential maximizing joint policy, treating it as a single-agent MDP, using a standard RL algorithm, e.g., value iteration, policy gradient, and assign individual policies to each agent \cite{littman1994markov,gonzalez2013discrete,zazo2016dynamic,macua2018learning}. In the absence of a centralized entity, if the goal is to attain a maximum of a common objective, e.g., the average reward of the agents, and this objective is commonly known, then the agents can act as a team. In such a setting, the agents can independently collect rewards and update their individual policies to maximize the common objective using a MARL method \cite{zhang2021multi}. 

\blue{A distinct and complementary form of coupling arises when an agent must 
coordinate against the \emph{strategies} the other agents are running, rather 
than react to their realized actions after the fact. The value of conditioning 
on others' strategies is well recognized: an agent that accounts for others' 
strategies coordinates and adapts substantially better than an independent 
learner that treats the other agents as a stationary part of the environment 
\cite{foerster2017learning,he2016opponent}. This is especially pronounced under 
commitment, when agents fix plans in advance and reacting to realized actions is 
too late.  In robotics, mobile robots and autonomous 
vehicles plan their routes and maneuvers against the routing and navigation 
strategies of the rest of the fleet to avoid congestion and deadlock, rather 
than replanning only after collisions materialize 
\cite{mason2023multi}. In supply chains, vendors coordinate replenishment 
timing to meet a shared demand while avoiding simultaneous over-supply, which 
requires anticipating the others' replenishment strategies rather than 
observing their shipments after the fact \cite{liu2025multi}. In each of 
these settings, the information that matters is not the current state or the 
realized actions alone, but the \emph{strategies} the other agents are 
running, which are encoded in their policy parameters.}

In this paper, we introduce a class of networked policy gradient algorithms, in which agents have parameterized policies that not just depend on the common state but also on others' policy parameters. Similar to the single-agent or independent policy gradient \cite{williams1992simple,sutton1999policy,zhang2020global,leonardos2021global}, the policy parameters are updated using local policy gradients which require two distinct sets of information as per the policy gradient theorem: (a) an estimate of the value of the current policy, and (b) score functions of all the local policies (local gradients of the log of the policies). Given the dependence of the local policies on others' policy parameters, agents need to maintain an estimate of all the other agents' policy parameters (even if they are not neighbors) in order to be able to execute their local policies, and compute the local gradients. We design an episodic learning scheme similar to \cite{zhang2020global} that consists of two consecutive episodes with random horizon lengths. In the first episode, agents sample their joint state-action pair to compute the score function, and starting from this sample, they collect discounted rewards through the second episode. After the local gradient updates, agents exchange their local estimates of parameters with their neighbors in a time-varying network, and update their local estimates of other agents' parameters. 

%to estimate the gradients by execution of individual policies against each other through two back-to-back episodes with random lengths of horizons. On par with the definition of policy gradients, in the first episode agents sample their joint state-action pair to compute the score function, and starting from this sample, they collect discounted rewards through the second episode. However, their policies need information on other agents' parameters even if they are not neighbors of each other in a communication network. In this case,  agents keep local estimates of other agents' parameters and update with the information coming from arising communication links changing over time. 



%After the early work on the usage of Markov games in MARL problems \cite{littman1994markov}, initial studies solving (constrained) Markov potential games with policy gradients analyze continuous state and action spaces with the assumption on twice differentiability of reward functions and/or state dynamics of agents \cite{gonzalez2013discrete,zazo2016dynamic,macua2018learning}. Their approach is to solve the game as a (centralized) single-agent problem using potential functions.

%Networked multiple decision-makers (agents) interact with each other in a system through a communication network. They share their information to improve decision-making capabilities. In this paper, we are interested in designing a networked multi-agent reinforcement learning (MARL) structure for individual decision-makers in dynamic states. 
%Networked MARL has shown success in handling important problems in different areas of engineering such as mobile robotics \cite{mason2023multi}, navigation \cite{kim2019learning}, and traffic management \cite{gupta2020networked} (see \cite{zhu2022survey} for an overview of networked MARL). This success in addition to the developments in single-agent RL, brings the question of the theoretical design for individual networked decision-makers. Game theory and game-theoretical learning provide a framework to answer this question.

%Markov (stochastic) \cite{shapley1953stochastic} games are a subclass of games that define the concept of individual decision-makers in dynamically evolving environments. In this setting, agents aim to maximize their individual utilities, depending on joint decisions. 
%More specifically, we formalize the concept of networked learning in Markov potential games, where a global potential function aligns with the changes in individual utilities. 

%We define a new class of policy learning structure by letting agents have policy functions based on information coming from other agents as input. We present a learning mechanism based on parameterized individual policies defined over the joint space of individual parameters, in which parameters are updated with policy gradients \cite{williams1992simple,sutton1999policy}. Using parameterized policies, agents map state information to the space of probability distributions over the action space of agents. The policy gradient estimation needs two distinct sets of information which are the estimated value of collected rewards and score functions of policies as probability distributions. We design episodic learning to estimate the gradients by execution of individual policies against each other through two back-to-back episodes with random lengths of horizons. On par with the definition of policy gradients, in the first episode agents sample their joint state-action pair to compute the score function, and starting from this sample, they collect discounted rewards through the second episode. However, their policies need information on other agents' parameters even if they are not neighbors of each other in a communication network. In this case,  agents keep local estimates of other agents' parameters and update with the information coming from arising communication links changing over time. 

We prove the convergence of \textit{networked policy gradient play} to a stationary point of the potential value function of the Markov  game almost surely (Theorem \ref{thm_as_con}) with iteration complexity $\ccalO({1}/{\epsilon^2})$ (Theorem \ref{thm_rate}). These results follow from four intermediate results. First, we show that policy gradients are Lipschitz continuous (Lemma \ref{lemma_lip}) and the episodic sampling provides an unbiased estimation of each agent's policy gradient (Lemma \ref{lem_unb}).  Next, we derive the convergence of local beliefs to the true parameter values in expectation (Lemma \ref{lemma_local_conv}). Lastly, we bound the potential value function changes over consecutive updates (Lemma \ref{lem_iter}). \blue{Numerical experiments on a dynamic multi-agent target assignment problem illustrate networked policies using time-varying networks with only $\mathcal{O}(1)$ transmissions per iteration attain higher rewards in comparison to communication-free local and independent policies, and a centralized-training baseline, namely proximal policy optimization (MAPPO) \cite{yu2022surprising}.}%, while their gradients converge to a stationary point of the potential function.  


% The paper is organized as follows. We first discuss the related literature in Section \ref{sec_lit}. We state the notation and the problem setting by defining Markov potential games in Section \ref{sec:main}. We present the algorithm in Section \ref{sec_learning}. We analyze the theoretical aspects of the proposed algorithm and show convergence in Section \ref{sec::conv}. We numerically assess the performance of the networked policy gradients against independent policy gradients as a baseline solution in Section \ref{sec:experiments}. Conclusions follow in Section \ref{sec:conclusions}.




%Our main results are in, our new algorithm is in , experimentalresults are in \cref{sec:experiments}, and the
%parameterization over finite state spaces. Based on the type of parameterization, agents use projected, standard, or natural policy gradient updates.

\vspace{-4pt}
\subsection{Related Literature and Contributions}
\label{sec_lit}
%After the early work on the usage of Markov games in MARL problems \cite{littman1994markov}, initial studies solving (constrained) Markov potential games with policy gradients \cite{gonzalez2013discrete,zazo2016dynamic,macua2018learning} analyze continuous state and action spaces with the assumption on twice differentiability of reward functions and/or state dynamics of agents. Their approach is to solve the game as a (centralized) single-agent problem using potential functions.
Following the terminology  in static games \cite{shamma2005dynamic}, we use \emph{policy gradient play} to refer to simultaneous policy-gradient
updates in which each agent ascends its own value function.  Distributed
variants using consensus have been studied for monotone games
\cite{tatarenko2020geometric,tan2024timestamp} and min--max problems
\cite{liu2022recursive}.

Independent policy-gradient methods have convergence guarantees for
structured Markov games, including potential and zero-sum games
\cite{zhang2024gradient,leonardos2021global,ding2022independent,
giannou2022convergence,fox2022independent,mao2022improving,
daskalakis2020independent,sun2023provably}.
For finite state and action spaces, these results exploit the game
structure and policy parameterization to relate stationarity to Nash
equilibrium. Direct parameterizations are studied in
\cite{zhang2024gradient,leonardos2021global}, while natural
policy-gradient methods are analyzed in
\cite{fox2022independent,ding2022independent}.
Extensions include linear $Q$-function approximation for infinite
spaces \cite{ding2022independent}, deterministic policies
\cite{giannou2022convergence}, and momentum-based variance reduction
\cite{mao2022improving}.
We instead study policies coupled through agents' parameters over
general, possibly infinite state and action spaces, with convergence
guarantees stated in terms of stationarity.

% In Markov games, independent policy gradient algorithms are shown to converge to a stationary NE by focusing on a particular utility structure, e.g. potential or zero-sum, with finite action and state spaces \cite{zhang2024gradient,leonardos2021global, ding2022independent, giannou2022convergence, fox2022independent, mao2022improving,daskalakis2020independent,sun2023provably}. The premise of the convergence to NE is established via the fact that stationary points of the gradients correspond to Nash equilibria when the state and action space is finite.  The works  \cite{zhang2024gradient,leonardos2021global} focus on direct parameterization and prove convergence to Nash Equilibrium (NE) for model-based and model-free settings. In \cite{fox2022independent,ding2022independent}, they show point-wise convergence with iteration complexity $\ccalO(1/\epsilon^2)$ using natural policy gradients. In \cite{ding2022independent}, the authors extend the finite state-action setting to the infinite case using linear function approximation of $Q$ functions showing convergence to an approximate NE. The work \cite{giannou2022convergence} concludes the convergence for deterministic policies. Similarly in \cite{mao2022improving}, the authors employ a momentum-based variance reduction method with policy gradients and obtain $\ccalO(1/\epsilon^{4.5})$ sample complexity bound. These works only focus on independent learning and consider finite and state actions to establish convergence to NE. We generalize their settings by considering networked policies and allowing the cardinality of state and action spaces to be infinite. 
Other networked MARL methods use consensus to estimate global value functions, $Q$-functions, or rewards \cite{yi2021learning,zhang2018fully,qu2019value}. A separate line combines fictitious play or best-response learning
with reinforcement learning, maintaining beliefs about other agents' policies in finite Markov games
\cite{sayin2022fictitious,baudin2022fictitious}.
Methods for networked MDPs instead exploit local transition structure, where each agent's next state depends on neighboring states and actions, using policy gradients \cite{lin2021multi} or policy iteration \cite{zhang2023global}. Our consensus process tracks other agents' policy parameters for use in coupled policies.
% There exist other networked MARL algorithms for solving multi-agent MDPs or Markov games that involve consensus updates   \cite{yi2021learning,zhang2018fully,qu2019value}. These algorithms use information exchanges along with consensus-type updates to better estimate the global value function or $Q$-function estimates in a distributed manner. 
% %Another relevant set of studies in solving Markov games are 
% Another related suite of MARL algorithms combine game-theoretic learning algorithms, e.g., fictitious play or best-response with standard RL algorithms, e.g., Q-learning \cite{sayin2022fictitious,baudin2022fictitious} that rely on agents having beliefs on others' policies in order to be able compute their best strategy from an estimated Q-function. These algorithms are suitable for and analyzed considering finite action and state spaces.
% Recent MARL algorithms for solving multi-agent MDPs with networked dynamics are also relevant \cite{lin2021multi,zhang2023global}. The setting assumes each agent has a local state that is affected by the neighbors' actions and states. The learning protocols proposed in this setting include variants of policy learning such as policy gradients \cite{lin2021multi}, and policy iteration \cite{zhang2023global}. %, while the authors prove convergence via exponential decay property. 
%Another line of work is similar to our setting, in terms of employing consensus updates within MARL. However, the difference is that agents use consensus processes to learn the parameters \cite{zhang2018fully,qu2019value} of global value functions or rewards \cite{yi2021learning} in a distributed optimization setting. An additional interesting study
%\cite{qu2020intention} models agents' joint policies as a neural network in networked Markov Decision Processes (MDP) where agents update individual intentions with message passing using Graph Neural Networks (GNN)s.


\blue{Our contributions and distinctions from prior work are as follows.

\noindent 1) \textit{Networked Policies and Gradient Estimation:}
We develop policy-gradient play for policies that depend on other agents' parameters, introducing cross-agent score terms absent from independent-policy methods.
We incorporate advantage and temporal-difference estimators and establish unbiasedness (Lemma~\ref{lem_unb}) and Lipschitz continuity (Lemma~\ref{lemma_lip}) under bounded-second-moment assumptions on the score functions. Compared with \cite{zhang2020global,aydin2023networked,aydin2023policyL4DC, aydin2023policy}, we relax almost-sure boundedness and account for baseline cancellation under cross-agent coupling.

\noindent 2) \textit{Consensus under Imperfect Information:}
We establish convergence of agents' beliefs about others' parameters under bounded-moment gradient estimates, admissible polynomially decaying stepsizes, and inaccurate initial beliefs (Lemma~\ref{lemma_local_conv}).
This relaxes the boundedness and initial-agreement assumptions in \cite{eksin2017distributed,arefizadeh2019distributed,
aydin2021decentralized}.

\noindent 3) \textit{Almost-Sure Convergence and Iteration Complexity:} We control the interaction between consensus errors and sampling noise to establish almost-sure convergence of networked policy-gradient play to stationarity of the potential value function (Theorem~\ref{thm_as_con}), strengthening the convergence-in-probability guarantees of
\cite{aydin2023policy,aydin2023networked,aydin2023policyL4DC}.
The method attains $\mathcal{O}(\epsilon^{-2})$ iteration complexity (Theorem~\ref{thm_rate}). For general state and action spaces, stationarity need not imply Nash equilibrium. 
}
% \noindent 1) \textit{Design of Networked Policies:} We devise stochastic gradient updates based on networked policies, which depend on other agents' parameters. The training phase involves consensus protocol for keeping track of other agents' parameters. We generalize the convergence result for the consensus protocol by allowing agents to start with incorrect initial beliefs. Numerical experiments demonstrate the potential for performance improvement by using networked policies instead of independent policies, while having similar or improved convergence rates.

% \noindent 2) \textit{Stochastic Gradient Estimation} We include alternative reward collection mechanisms, e.g., advantage function and temporal difference, that are used in estimating the stochastic gradient. We establish the Lipschitz continuity (Lemma \ref{lemma_lip}) and unbiasedness (Lemma \ref{lem_unb}) of the policy gradient estimators assuming only bounded second moments of the score functions.


% % We propose a policy gradient estimation method (Algorithm~\ref{alg_est_inner}) under different reward collection mechanisms, e.g., advantage function and temporal difference. In addition, we establish the Lipschitz continuity (Lemma \ref{lemma_lip}) and unbiasedness (Lemma \ref{lem_unb}) of the policy gradient estimators assuming only bounded second moments of the score functions.

% % \noindent 2) \textit{Consensus of Beliefs:} We prove that the belief exchange on other agents' parameters converges to the true parameter values in expectation (Lemma~ \ref{lemma_local_conv}). Our result extends prior works by relaxing the assumptions of almost surely bounded policy gradient estimators, generalizing the decay rates of stepsizes, and removing the requirement of perfect knowledge of the initial parameter values among agents.

% \noindent 3) \textit{Almost Sure Convergence and $\mathcal{O}(\epsilon^{-2})$ iteration complexity:} We prove that the \textit{networked policy gradient play} (Algorithm~\ref{alg_DFP}) converges almost surely to a stationary point of the potential value of the Markov game (Theorem~\ref{thm_as_con}), with iteration complexity  $\mathcal{O}(\epsilon^{-2})$ (Theorem~\ref{thm_rate}). %When the state and action spaces are not finite, the stationary points of the potential value function is not guaranteed to be a NE. Hence, we attain convergence to an approximate NE. 
% The iteration complexity matches the complexity established for stochastic gradient and independent policy gradient algorithms, e.g., see \cite{ding2022independent}. 

% \blue{This paper addresses challenges absent in relevant single-agent methods \cite{zhang2020global} or our prior work \cite{aydin2023policy,aydin2023networked,aydin2023policyL4DC}. We summarize the distinct challenges addressed below:}

% \noindent $\bullet$ \textit{Design of Networked Policies:} We devise stochastic gradient updates based on networked policies, which depend on other agents' parameters. \blue{This parameterization introduces cross-agent score terms into the policy gradient that are absent in the single-agent setting of \cite{zhang2020global} and in independent-policy methods. In contrast to prior versions \cite{aydin2023networked,aydin2023policyL4DC,aydin2023policy}, which considered only a plain policy gradient without baseline functions, we incorporate baseline-based estimators, including the advantage and temporal-difference variants.} %The training phase involves a consensus protocol for keeping track of other agents' parameters. Numerical experiments show improved reward collection when networked policies are used instead of local or independent policies.

% \noindent $\bullet$ \textit{Gradient Estimation:} We include alternative reward collection mechanisms, e.g., advantage function and temporal difference, that are used in estimating the stochastic gradient. We establish the unbiasedness (Lemma~\ref{lem_unb}) and Lipschitz continuity (Lemma~\ref{lemma_lip}) of the policy gradient estimators assuming only bounded second moments of the score functions\blue{, rather than the almost-sure boundedness required in \cite{zhang2020global,aydin2023networked,aydin2023policyL4DC,aydin2023policy}. This relaxation admits policy classes with unbounded action support, such as Gaussian policies, that almost-sure boundedness excludes. Establishing unbiasedness requires showing that baseline functions preserve it under the cross-agent coupling, and Lipschitz continuity must account for the belief errors generated by the communication process, neither of which arises in \cite{zhang2020global}.}

% \blue{\noindent $\bullet$ \textit{Consensus of Beliefs:} Lemma~\ref{lemma_local_conv} establishes belief convergence under
% bounded-moment policy-gradient estimates, general polynomially decaying stepsizes, and potentially inaccurate initial beliefs, thereby relaxing the boundedness and initial-agreement assumptions of prior work \cite{eksin2017distributed,arefizadeh2019distributed, aydin2021decentralized}.}

% \blue{\noindent $\bullet$ \textit{Almost-Sure Convergence with Matching
% Complexity:}
% Belief-estimation errors induced by time-varying communication enter the gradient recursion as perturbations coupled with the sampling noise. We develop a joint consensus-and-learning argument establishing that these perturbations are summable. This strengthens the convergence-in-probability guarantees of our prior work \cite{aydin2023policy,aydin2023networked,aydin2023policyL4DC} to almost-sure convergence, while attaining the same $\mathcal{O}(\epsilon^{-2})$ complexity as standard stochastic-gradient and independent-policy-gradient methods \cite{ding2022independent}. For general, possibly infinite state and action spaces, stationary points need not be Nash equilibria; accordingly, our guarantee is stated in terms of stationarity.}


% Unlike our previous studies \cite{aydin2023networked,aydin2023policyL4DC,aydin2023policy}, we prove the result  even though belief errors vanish in expectation, which violates standard supermartingale properties.
% , their expected cumulative sum is convergent and local belief errors converge almost surely.

 
% Our previous work on networked policy gradients \cite{aydin2023policy,aydin2023networked,aydin2023policyL4DC} is limited to stepsizes proportional to $1/t$, $Q$-function-based gradient estimators, and convergence in probability under almost-sure boundedness of policy score functions and exact initial agreement among agents. Here, we consider more general polynomially decaying stepsizes, incorporate advantage- and temporal-difference-based estimators, and establish almost-sure convergence under bounded first and second moments of the score functions and potentially inaccurate initial beliefs. Numerical results further demonstrate that the advantage and temporal-difference estimators improve performance and stability.
% In contrast to \cite{zhang2020global} and our prior works \cite{aydin2023policy,aydin2023networked,aydin2023policyL4DC} that assume bounded score functions of the policies, we assume only the expectations and second moments of the score functions are bounded (Assumption \ref{as_bound_logp}) in proving unbiasedness.
%\lipsum[2-3]

% The outline is not required, but we show an example here.


==> dfp_com_aware/my_sections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> dfp_com_aware/results_learning_dynamics.tex <==
% !TEX root = Control in state-based anti-coordination network games.tex

\subsection{Game theoretic preliminaries}
We consider the  Nash equilibrium solution concept as a rational action profile. A Nash equilibrium (NE) $a^{\text{NE}} \in [0,1]^n$ is an action profile that satisfies
%
\begin{align} \label{Nash_definition}
u_i(a_i^{\text{NE}}, a_{\ccalN_i}^{\text{\text{NE}}}) \geq  u_i(a_i, a_{\ccalN_i}^{\text{NE}}) \quad a_i \in [0,1], i \in \ccalN
\end{align}
%
% where $a_{\ccalN_i}^{\text{NE}} := \{a_{j}^{\text{NE}}: j\in \ccalN_i \}$.
%
In other words, the individuals best-respond to the NE actions of other individuals. For a given neighbor action profile $a_{\ccalN_i}$ the best response for player $i$ is
%
\begin{align}
BR_i(a_{\ccalN_i}) &:= \argmax_{a_i \in [0,1]} u_i(a_i, a_{\ccalN_i}) \label{best_response} \\
& = \bbone\left({1} >  (c_0 (1-s_i)+c_1 s_i) \sum_{j\in \ccalN_i} a_j \right) \label{best_response_specific}
\end{align}
%
where $\bbone(\cdot)$ is an indicator function. Since the payoffs are linear in self-actions, the actions that maximize the payoffs are in the extremes---$a_i =1$ or $a_i = 0$---depending on the types and actions of their neighbors. 
We can equivalently represent the NE definition in \eqref{Nash_definition} by using the best response definition,  
%
\begin{align} \label{NE_best_response}
a_i^{\text{NE}} = BR_i(a_{\ccalN_i}^{\text{NE}}) \quad \forall i\in \ccalN.
\end{align}
%

The notion of strictly dominated is defined in the following.

%
\begin{definition}[Strictly dominated action] \label{strictly_dominated_definition}
An action $a_i \in [0,1]$ is strictly dominated if and only if there exists an action $a_i' \in [0,1]$ such that 
\begin{equation}\label{eq:strictly_dominated_definition}
u_i(a_i', a_{\ccalN_i}) >  u_i(a_i, a_{\ccalN_i}) \quad \forall a_{\ccalN_i}\in \ccalA_{\ccalN_i}.
\end{equation}
\end{definition}
%
If an action $a_i$ is strictly dominated then there exists a more preferable action $a_i'$ for any circumstance. From \eqref{NE_best_response}, a strictly dominated action cannot be rational .
%
%\red{The algorithm is based on the iterated elimination process in which the dominated actions are eliminated in a sequential manner. }
%\red{In the following we define a strictly dominated action which will be a useful concept in finding the Nash equilibrium. }

In the game $\Gamma$, we can iteratively remove the strictly dominated actions. This process is called the iterated elimination of strictly dominated strategies, defined below.
%
\begin{definition}[Iterated elimination] \label{def:elimination_strict}
Set the initial set of actions $A_i^0 = [0,1]$ for all $i$, and for any $k\in \naturals$ let 
\begin{equation}
	\begin{aligned}
	A_i^k = \{a_i \in &A_i^{k-1} \given \\
	&a_i \text{ is not strictly dominated by any } a_{\ccalN_i} \in A_{\ccalN_i}^{k-1}\}.
	\end{aligned}
\end{equation}
%	
\end{definition}
%
We denote the set of player $i$'s actions that survive the iterated elimination by $A_i^\infty := \bigcap_{k =0}^\infty A_i^k$. If $A_i^\infty$ is a singleton (has a single element) for all $i\in\ccalN$, then the game is dominance solvable, and has a unique Nash equilibrium given by the action profile that survives the iterated elimination process. 
%
\subsection{Convergence}
%

%\section{Finite time Nash equilibrium learning}
%We define the rational action in the stage game by the Nash equilibrium solution concept. A Nash equilibrium (NE) action profile $a^{NE} \in [0,1]^n$ is such that no individual has a preferable deviation from its action, that is, for a given state $s$,
%%
%\begin{align} \label{Nash_definition}
%u_i(a_i^{NE}, a_{\ccalN_i^C}^{NE}, s_i, s_{\ccalN_i^C}) \geq  u_i(a_i, a_{\ccalN_i^C}^{NE}, s_i, s_{\ccalN_i^C}) \quad a_i \in [0,1],  \forall i \in \ccalN
%\end{align}
%%
%where $a_{\ccalN_i^C}^{NE} := \{a_{j}^{NE}: j\in \ccalN_i^C \}$.
%%
%In other words, the individuals respond to the NE actions of other individuals to maximize their payoffs. For a given state $s_i, s_{\ccalN_i^C}$ and neighbor action profile $a_{\ccalN_i^C}$ we have the best response of individual $i$ as follows,
%%
%\begin{align}
%BR_i(a_{\ccalN_i^C}, s_i, s_{\ccalN_i^C}) &:= \argmax_{a_i \in [0,1]} u_i(a_i, a_{\ccalN_i^C}, s_{\ccalN_i^C})) \label{best_response} \\
%& = \bbone\left({1} > \beta c_0 (1-s_i) \sum_{j\in \ccalN_i^C} a_j s_j + {\beta c_1 s_i \sum_{j\in\ccalN_i^C} a_j (1-s_j)}\right) \label{best_response_specific}
%\end{align}
%%
%where $\bbone(\cdot)$ is an indicator function. Since the payoffs are linear in self-actions, the actions that maximize the payoffs are in the extremes -- $a_i =1$ or $a_i = 0$ -- depending on the states and actions of their neighbors. 
%We can equivalently represent the NE definition in \eqref{Nash_definition} by using the best response definition,  
%%
%\begin{align} \label{NE_best_response}
%a_i^{NE} = BR_i(a_{\ccalN_i^C}^{NE}, s_i, s_{\ccalN_i^C}) \quad \forall i\in \ccalN.
%\end{align}
%%
%In the following we define a strictly dominated action which will be a useful concept in finding the Nash equilibrium. 
%%
%\begin{definition}[Strictly dominated action] \label{strictly_dominated_definition}
%An action $a_i \in [0,1]$ is strictly dominated if and only if there exists an action $a_i' \in [0,1]$ such that 
%\begin{equation}\label{eq:strictly_dominated_definition}
%u_i(a_i', a_{\ccalN_i^C}, s_i, s_{\ccalN_i^C}) >  u_i(a_i, a_{\ccalN_i^C}, s_i, s_{\ccalN_i^C}) \quad \forall a_{\ccalN_i^C}
%\end{equation}
%\end{definition}
%%
%If an action $a_i$ is strictly dominated then there exists a more preferable action $a_i'$ for any circumstance. It is clear that if an action is strictly dominated then it cannot be a rational action from \eqref{NE_best_response}. In a game we can iteratively remove the strictly dominated actions, this process is called the iterated elimination of strictly dominated strategies and is defined below.
%%
%\begin{definition}[Iterated elimination of strictly dominated actions] \label{def:elimination_strict}
%Set the initial set of actions $A_i^0 = [0,1]$ for all $i$, and for any $k\in \naturals$ set 
%\begin{equation}
%A_i^k = \{a_i \in A_i^{k-1} \given a_i \text{ is not strictly dominated given any } a_{\ccalN_i^C} \in A_{\ccalN_i^C}^{k-1}\}
%\end{equation}
%\end{definition}
%%
%We denote the set of actions of individual $i$ that survive the iterated elimination by $A_i^\infty := \bigcap_{k =0}^\infty A_i^k$. When $A_i^\infty$ has a single element, we say $A_i^\infty$ is a singleton. Inspired by the process above, we propose the following local algorithm. 

%\begin{definition}[Local algorithm] \label{local_algorithm}
%Given state $s \in \{0,1\}^n$. Initially set $a_{i,0} = \epsilon$ where $1>\epsilon>0$.  At each iteration $k \in \naturals$, if $a_{i, k-1} \in \{0,1\}$, set $a_{i,k} =a_{i, k-1}$. Otherwise, observe neighbors actions $a_{\ccalN_i^C, k-1}$. If $a_{j, k-1} = a_{j, k-2} =\dots = a_{j, k-n}$ for all $j \in \ccalN_i^C$ when $k \geq n$ then select $a_{i, k} = 1$ if $s_i =0$ or $a_{i, k} = 0$ if $s_i =1$. Otherwise, update $a_{i, k}$ as follows
%%For all $j \in \ccalN_i^C$ define $a'_j = a_{j, k-1}$ if $a_{j, k-1} \in \{0,1\}$, otherwise $a'_j = 1$ when $k$ is odd and $a'_j = 0$ when $k$ is even. Then for $k$ odd, 
%%
%\begin{align} \label{worst_case_good_response_2}
%a_{i,k} = 1 \quad\text{ if } 1 > \beta (c_0 (1-s_i) \sum_{j\in \ccalN_i^C} \left\lceil a_{j,k-1} \right\rceil s_j +  c_1 s_i \sum_{j\in\ccalN_i^C} \left\lceil a_{j,k-1} \right\rceil (1-s_j)),
%\end{align}
%%
%%
%\begin{align} \label{best_case_bad_response_2}
%a_{i,k} = 0 \quad\text{ if } 1 < \beta (c_0 (1-s_i) \sum_{j\in \ccalN_i^C} \lfloor a_{j,k-1} \rfloor s_j + c_1 s_i \sum_{j\in\ccalN_i^C} \lfloor a_{j,k-1} \rfloor(1-s_j))
%\end{align}
%%
%where $\lceil \cdot \rceil$ is the ceil function and $\lfloor \cdot \rfloor$ is the floor function. Otherwise, select $a_{i,k} = \epsilon$. Share $a_{i,k}$ with $j \in \ccalN_i^C$. If $k<2n$, advance the iteration number $k = k+1$.
%\end{definition}

%
%The algorithm above is local, only relies on observing actions of one's neighbors in the network. The update in \eqref{worst_case_good_response} is a \emph{socialize} response to a worst case scenario where besides neighbors that have actions $a_{j,k-1} = 0$, every $j \in \ccalN_i^C$ is considered to be socializing with interaction level 1. Even in this worst possible scenario, if the socializing constant $1$ is larger than the right hand side of the condition in \eqref{worst_case_good_response} then individual $i$ selects to socialize fully. In contrast, the update in \eqref{best_case_bad_response} is a \emph{do not socialize} response to a best case scenario where besides neighbors that announce to socialize fully $a_{j,k-1} = 1$, every $j \in \ccalN_i^C$ is considered to be isolated off from the network. Even in this best possible scenario, if the socializing constant $1$ is smaller than the right hand side of the condition in \eqref{best_case_bad_response} then individual $i$ selects to isolate itself by selecting $a_{i,k} = 0$. If none of the two conditions in \eqref{worst_case_good_response} and \eqref{best_case_bad_response} is satisfied, then the individual makes a provisional social interaction decision of $1>\epsilon >0$. We exemplify this algorithm on a simple  network in an illustration -- see Figure \ref{fig:algorithm_example}. 

The following theorem states that Algorithm \ref{local_alg} eliminates all strictly dominated actions in finite number of steps.

%\begin{theorem} \label{local_algorithm_convergence}
%Algorithm \ref{local_alg} converges in at most $n$ iterations, that is, no player changes its action after the $n$th update. At the end of $n$ iterations, if all players are decided, i.e., $a_{i}^n = \{0,1\}$ for all $i\in\ccalN$, then all the other actions $\ccalA_i \setminus a_{i}^n$ are strictly dominated and the resultant action profile is a Nash equilibrium. Otherwise, if a player $i \in \ccalN$ is undecided, i.e., $a_{i}^n = \epsilon$, then there does not exist $a_i \in \ccalA_i$ that can be strictly dominated. 
%\end{theorem}
\begin{theorem} \label{local_algorithm_convergence}
Assume all players are undecided, i.e., $a_{i}^0 = \epsilon$ for $i\in\ccalN$. Algorithm \ref{local_alg} converges in at most $n$ iterations, that is, no player changes its action after the $n$th update. If all players are decided, i.e., $a_{i}^n = \{0,1\}$ for all $i\in\ccalN$, the resultant action profile $a^n$ is a Nash equilibrium. Otherwise, if a player $i \in \ccalN$ is undecided, then there does not exist $a_i \in \ccalA_i$ that can be strictly dominated. 
\end{theorem}

%
%
%if all players are decided, i.e., $a_{i,n} = \{0,1\}$, then the resulting action profile $a \in \ccalA$ is the unique Nash equilibrium. 
%
%In Algorithm \ref{local_alg}, no updates are possible after
%
%if all players are decidd
%
% converges to a pure Nash equilibrium of the game with payoffs given by  \eqref{utility} in $n$ steps. 
%

The proof (see Appendix) relies on showing that Algorithm \ref{local_algorithm_convergence} is a decentralized version of the iterated elimination of strictly dominated actions as given by Definition \ref{def:elimination_strict}. The intuition for $n$ step convergence is that at each step at least one player needs to eliminate its action using \eqref{worst_case_good_response} or \eqref{best_case_bad_response}. If no player updates at a time step, the players stop updating because no new eliminations are triggered. Therefore, there could  at most be $n$ iterations to rule out $n$ players one player at a time.




